Analyzing and Adapting Large Language Models for Few-Shot Multilingual NLU: Are We There Yet?

Supervised fine-tuning (SFT), supervised instruction tuning (SIT) and in-context learning (ICL) are three alternative, de facto standard approaches to few-shot learning. ICL has gained popularity recently with the advent of LLMs due to its simplicity and sample efficiency. Prior research has conducted only limited investigation into how these approaches work for multilingual few-shot learning, and the focus so far has been mostly on their performance. In this work, we present an extensive and systematic comparison of the three approaches, testing them on 6 high- and low-resource languages, three different NLU tasks, and a myriad of language and domain setups. Importantly, performance is only one aspect of the comparison, where we also analyse the approaches through the optics of their computational, inference and financial costs. Our observations show that supervised instruction tuning has the best trade-off between performance and resource requirements. As another contribution, we analyse the impact of target language adaptation of pretrained LLMs and find that the standard adaptation approaches can (superficially) improve target language generation capabilities, but language understanding elicited through ICL does not improve and remains limited, with low scores especially for low-resource languages.

==> introduction_in_ashes.tex <==
Multilingually pretrained language models (termed \textit{mPLMs} henceforth) \ivan{Does this subsume LLMs or it's only encoder-only models?} have a pivotal role in steering, increasing and promoting language inclusiveness of NLP technology \cite{devlin-etal-2019-bert, conneau-etal-2020-unsupervised, imanigooghari-etal-2023-glot500}. Due to a wide range of languages included in their pretraining, mPLMs have been used for cross-lingual transfer and sample-efficient adaptation to many languages of the world, including both languages seen \cite{wu-dredze-2019-beto, wu-dredze-2020-languages} and unseen \cite{winata-etal-2022-cross} during pretraining. One common approach to adapt an mPLM for a given task-language combination is via \textit{Supervised Fine-Tuning (SFT)} where the mPLM is finetuned on a downstream task, either directly for a target language (CITE), or via zero-shot (CITE) or few-shot cross-lingual transfer from a source language with more abundant task data (CITE). \ivan{We have to be careful here - this claim somehow contradicts the ideas of cross-lingual transfer? We need to structure the argument here very carefully.} 

While SFT in such setups has achieved state-of-the-art (SoTA) performances for plethora of target language-task combinations, it has at least two major downsides: \textbf{1)} SFT yields a model specialised for a single \textit{language-task} combination which can be intractable when a large number of languages and/or tasks have to be covered;\ivan{But this downside is mitigated via modular designs? Again, we need to refine the argument a bit} and \textbf{2)} SFT necessitates expensive and complex data collection in the target language, which can be especially challenging for low-resource languages.
\ivan{Figure 1 critically needs redesign of the labels, especially the ones around the radar edges!}
\genie{is the current one any better? with just white background?}

\begin{figure}[!t]
\centering
\begin{subfigure}[b]{0.35\textwidth}
   \includegraphics[width=1\linewidth]{images/id_practical_comparisons_amh.png}
   \caption{Amharic}
   \label{fig:comparison_practicalities_amh} 
\end{subfigure} \quad
\begin{subfigure}[b]{0.35\textwidth}
   \includegraphics[width=1\linewidth]{images/id_practical_comparisons_es.png}
   \caption{Spanish}
   \label{fig:comparison_practicalities_es}
\end{subfigure}

\caption{Comparison of practical aspects of different learning paradigms for intent detection for Amharic and Spanish. ICL has low performance and high inference and computational costs while being comparatively cheap. SFT and SIT, on the other hand, have larger financial cost but they are much more efficient in terms of inference and computational resources while also being much more performant both for low (\ref{fig:comparison_practicalities_amh}) and high (\ref{fig:comparison_practicalities_es}) resource languages.}\label{fig:comparison_practicalities}
\end{figure}

Pretrained Large language models (LLMs) have played a pivotal role in modern NLP due to their general-purpose nature that yields strong performance across a wide range of tasks, indicating data efficiency. Using these models as a starting point, one can achieve better results on a given task with limited annotated data \citep{liu2022few-ia3}. Recently proposed multilingually pretrained language models (mPLM; CITE CITE) have demonstrated the same trends for cross-lingual transfer. A standard approach is supervised finetuning (SFT) where the mPLM is used for initialisation and then its parameters are updated on a downstream task for a target language. One downside of SFT is that for every \textit{task-language} combination one needs to tune a separate model on a separate training set which can be impractical when scaling to many languages or tasks.


An alternative approach which became popular with the advent of large language models (LLMs) such as GPT-4 \citep{achiam2023gpt4technical} and LLaMa-2 \citep{touvron2023llama2} is In-Context Learning (ICL), where, given an explanation of a task (i.e., \textit{instruction}) and a set of `training' examples (i.e., annotated \textit{demonstrations}), the model is tasked to generate the label for every input \citep{radford2019-in-context-learning}. ICL has shown great potential, achieving high performance on a variety of standard NLP tasks in English with only a handful of annotated examples \cite{dong2022survey-icl}. 

One benefit of ICL is that it does not require tuning the model to a specific task or language allowing the use of a single model to perform multiple tasks. In other words, ICL relies fully on the model's language capabilities learnt during pretraining. Pretraining of most LLMs is conducted in an English-centric manner where the vast majority of the pretraining corpus is in English with only limited coverage of other languages \cite{sitaram2023everything}, with even accidentally encountered bilingual and translation data \citep{briakou-etal-2023-searching}. As a result, current LLMs do not serve the world's languages equally: while demonstrating impressive ICL results in English \citep{mishra2022cross}, they still face difficulties when transferring to other languages \citep{winata2021language},\ivan{Do we have a better reference for this than the 2021 work?} especially the low-resourced ones \citep{ojo2023good}.\ivan{We should also cite some work that tried to adapt them multilingually somewhere, e.g., https://arxiv.org/abs/2204.07580, https://arxiv.org/abs/2401.01854}


There has been little attention drawn to which of the two techniques -- SFT or ICL --  works better in multilingual and cross-lingual settings in practice. Therefore, this paper aims to delve deeper into analysing a variety of factors which critically impact effective use of either approach from a more practical aspect. Our first aim is to provide answers to the following question:

\vspace{0.4mm}
\noindent \textit{(Q1) Given the same number of annotated examples, which of the two approaches -- SFT or ICL -- is better \textbf{in practice}?}
\vspace{0.4mm}

\noindent In particular, the term `practice' in our work comprises the following crucial aspects: \textbf{1)} sample efficiency (i.e., \textit{`data cost'}); \textbf{2)} computational requirements (\textit{`computational cost'}); \textbf{3)} latency (\textit{`inference cost'}); and \textbf{4)} overall financial or `economic' cost. Prior work has been mainly focused on benchmarking ICL on subgroups of languages \cite{ojo2023good} and only considered and optimised task performance of the models as the ultimate comparison criterion. In contrast, our work presents an extensive analysis evaluating cross-lingual capabilities of SFT and ICL both on high and low-resource languages, considering not only the task performance but also the above listed practical aspects.

%such as: a) sample efficiency; b) computational requirements; c) latency; and d) cost of each of the approaches. 

Furthermore, prior work has demonstrated the effectiveness of parameter-efficient fine-tuning (PEFT) to improve the model's cross-task capabilities and to promote aspects of its generation abilities (e.g., open-domain chat; \citeauthor{dettmers2023qlora}, \citeyear{dettmers2023qlora}). In this work, we also analyse how language adaptation of LLMs `beyond English' impacts their NLU and NLG performance in a target language.\ivan{Will we also provide some results testing their NLG capabilities?} This gives rise to another core research question:

\vspace{0.4mm}
\noindent \textit{(Q2) Given the benefits of ICL as a learning paradigm (but its inferior performance in comparison to SFT), could we use the standard adaptation strategies to improve the LLMs generation and understanding capabilities in other languages?}
\vspace{0.4mm}

\noindent The main focus of our analyses, revolving around Q1 and Q2, is on Natural Language Understanding (NLU) tasks\ivan{We say that we'll test generation and understanding capabilities, and then we say that the focus is on NLU tasks - this argument must be refined here} for task-oriented dialogue as one widely used and established practical application of NLP technology, due to multiple reasons. \textbf{1)} Dialogue is a user-facing application where computational and memory requirements, data collection cost, inference latency and other practical concerns are of ultimate importance. \textbf{2)} Dialogue NLU tasks provide well-defined ontologies and evaluation setups, with evaluation benchmarks that comprise comparable and semantically aligned training and test data across multiple languages, including high- and low-resource ones (CITE, CITE). \textbf{3)} In contrast to standard `non-dialogue' NLU tasks, dialogue NLU datasets are unlikely to have been `seen` by LLMs during their pretraining, which avoids test data leakage (CITE: papers on data contamination). \ivan{But we also do XNLI, what about testing generation?} \ivan{This whole paragraph discussing Dialogue NLU tasks is too verbose for the intro and should be put in the experimental setup.}

%\noindent \textit{(Q2) Given the benefits of ICL as a learning paradigm but its inferior performance in comparison to SFT, could we use the standard adaptation strategies to improve the LLMs understanding capabilities in other languages?}

%Prior work has demonstrated the effectiveness of parameter-efficient fine-tuning (PEFT) to improve the model's cross-task capabilities and to promote aspects of its generation abilities (e.g., open-domain chat; CITE: QLORA). In this work we analyse how language adaptation of LLMs influences their NLU performance in a target language. 

\rparagraph{Contributions}
\textbf{1)} We conduct a comprehensive analysis of in-context learning versus supervised fine-tuning paradigms in the context of multilingual few-shot adaptation, with the focus on multiple practical angles and cost. Our analyses demonstrate that not only the SFT approaches with smaller models lead to improved task performance but also they remain more data-, computation-, inference- and cost-effective than ICL with general-purpose LLMs. \textbf{2)} We investigate the effectiveness of target language adaptation, borrowed from the work on mPLMs, for ICL with LLMs.The main finding is that language adaptation leads to superficially improved generation capabilities in the target language with only limited improvements on the actual tasks, calling for further research that will mitigate the large language gap in LLM development and deployment between English and other languages. 









===================================================================

\begin{table}[!t]
\def\arraystretch{0.81}
{\fontsize{6.9}{7.1}\selectfont
%\footnotesize
%\resizebox{\linewidth}{!}{%
\begin{tabularx}{0.99\linewidth}{l YYYY}
\toprule
 \multirow{5}{*}{{\bf Language}} \\
 \multirow{2}{*}{{\bf Model}} & \multicolumn{2}{c}{\textsc{banking}} & \multicolumn{2}{c}{\textsc{hotels}} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5}
                      & \textit{20-Fold}    & \textit{10-Fold}   & \textit{20-Fold}    & \textit{10-Fold}   \\ \midrule
Non-tuned                     &     21.91       &     21.93     &  20.85     &     21.94     \\
Tuned for VE                   &        26.28         &   26.85        &   30.77         &    33.39      \\ \bottomrule
\end{tabularx}
}
\vspace{-1mm}
\caption{\method's (\textit{Desc.} cross-task transfer performance on NLU++; VE$\rightarrow$ID.}\label{tab:cross task}
\vspace{-1.5mm}
\end{table}














